A collision model for very flexible Cosserat rods and immersed-boundary fluid-structure coupling

The paper presents a constraint-based collision model for Cosserat rods, able to handle dynamic or static contact between a large number of highly flexible structures. The model provides the required collision impulses prior to updating the solution of the rods, with the impulses accounted for as external loads. The procedure avoids the need to modify the structure solver itself and circumvents any iteration between the collision model and the solver for the Cosserat rods, maintaining the efficiency of any chosen Cosserat solver. The collision model is adopted from Tschisgale et al. (Arch. Appl. Mech., 2019) and extended towards higher stability, which is found necessary in the case of very flexible rods. Furthermore, the model is supplemented with additional terms that arise when the colliding rods are immersed in a fluid. The latter is accounted for by an immersed-boundary method. A large number of tests are conducted to demonstrate the functionality of the final model.

==> latexmkrc <==
$makeindex = 'makeindex %.nlo -s nomencl.ist -o %.nls';
# Custom dependency and function for nomencl package 
add_cus_dep( 'nlo', 'nls', 0, 'makenlo2nls' );
sub makenlo2nls {
  system("makeindex -s nomencl.ist -o \"$_[0].nls\" \"$_[0].nlo\"");
}


==> nomenclature/customcommands.tex <==
%\usepackage{relsize}

%%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%% Gray rectangle to illustrate the use of modifiers and indices
%%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%\usepackage{stix} % provides \vrectangleblack, but clashes with other packages
%\usepackage{ifsym}
%\newcommand{\vgbox}{\text{\textcolor{gray}{\FilledSmallSquare}}}

%\DeclareFontFamily{U}{MnSymbolC}{}
%\DeclareFontShape{U}{MnSymbolC}{m}{n}{
%	<-5.5> MnSymbolC5
%	<5.5-6.5> MnSymbolC6
%	<6.5-7.5> MnSymbolC7
%	<7.5-8.5> MnSymbolC8
%	<8.5-9.5> MnSymbolC9
%	<9.5-11.5> MnSymbolC10
%	<11.5-> MnSymbolCb12
%}{}
%\DeclareRobustCommand{\gsqcdot}{%
%	\mathbin{\text{\color{gray}\usefont{U}{MnSymbolC}{m}{n}\symbol{"69}}}%
%}

%\newcommand{\gsqcdot}{\text{\color{gray}\filledsquare}}

%%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%% Some custom commands
%%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

\newcommand{\describevector}[1]{$\vectorsym{#1} = \transposed{(#1_x, #1_y, #1_z)}$}

%\newcommand{\SymbolForIllustrationOfScripts}{\cdot}
%\newcommand{\SymbolForIllustrationOfScripts}{(\cdot)}
\newcommand{\SymbolForIllustrationOfScripts}{\raisebox{-1pt}{$\color{gray}\blacksquare$}}
\newcommand{\wildcard}{\cdot}
\newcommand{\pwildcard}{(\cdot)}

%\DeclareMathAlphabet{\mathsfit}{T1}{\sfdefault}{\mddefault}{\sldefault}
%\SetMathAlphabet{\mathsfit}{bold}{T1}{\sfdefault}{\bfdefault}{\sldefault}
\newcommand{\s}{\mathrm{s}}
%\newcommand{\ssymbol}[1]{#1}
%\newcommand{\Deltadiff}[1]{{\Delta\!\!\:#1}}

% Commands for 2-column nomenclature layout
%\renewcommand*{\nompreamble}{\begin{multicols}{2}}
%	\renewcommand*{\nompostamble}{\end{multicols}}
%\setlength{\columnseprule}{0.4pt}

\newcommand{\ssymbol}[1]{\mathsfit{#1}}

% https://tex.stackexchange.com/a/712336/63717
\usepackage{amsmath,mathtools}
\DeclarePairedDelimiter{\anglebrackets}{\langle}{\rangle}
\NewDocumentCommand{\lrangles}{some{_^}}{%
  \IfBooleanTF{#1}{% *
    \anglebrackets*{#3}%
    \IfValueT{#4}{_{\!#4}}% subscript
    \IfValueT{#5}{^{\!#5}}% superscript
  }{%
    \IfNoValueTF{#2}{%
      \anglebrackets{#3}%
      \IfValueT{#4}{_{#4}}% subscript
      \IfValueT{#5}{^{#5}}% superscript
    }{%
      \anglebrackets[#2]{#3}%
      \IfValueT{#4}{_{\!#4}}% subscript
      \IfValueT{#5}{^{\!#5}}% superscript
    }%
  }%
}


% =======================================================

\newcommand{\structureelement}{n}
\newcommand{\collisionelement}{n}
\newcommand{\masterelement}{n}
\newcommand{\markerelement}{l}
\newcommand{\relstructureelement}[2]{\relelement{#1}{#2}}
\newcommand{\relcollisionelement}[2]{\relelement{#1}{#2}}
\newcommand{\relmarkerelement}[2]{\relelement{#1}{#2}}
\renewcommand{\gravityforcedensity}{\relgravity{\externalforcedensity}}
\newcommand{\bladekOne}{\bladeks{1}}
\newcommand{\bladekTwo}{\bladeks{2}}
\newcommand{\rkstep}{r}
%\introducerelrkstep
%\newcommand{\jpdf}[2]{\pdf{#1,#2}}
%\newcommand{\forcingmass}{\tilde{m}}

\newcommand{\collisionelementmass}{\relcoll{\mass}}
\newcommand{\markermass}{\relmarker{\mass}}


\newcommand{\frictionvelocityvo}{\relvo[\!,]{{\frictionvelocity}}}
\newcommand{\roughnessfunctionvo}{\relvo{\roughnessfunction}}
\newcommand{\viscouslengthvo}{\relvo{{\viscouslength}}}
\newcommand{\Reynoldsvo}{\relvo[\!,]{{\Reynolds_\tau}}}
\newcommand{\yplus}{y^+}

\newcommand{\imag}{\mathrm{i}}
\newcommand{\e}{\mathrm{e}}

\newcommand{\x}{\centerlinepos_x}
\newcommand{\y}{\centerlinepos_y}
\newcommand{\z}{\centerlinepos_z}
\newcommand{\negcorrxy}{-\corr{\tfl{\x}}{\tfl{\y}}}
\newcommand{\turbfrequency}{f\ind{t}}
\newcommand{\flapfrequency}{f\ind{f}}

\newcommand{\xhull}{x\ind{h}}
\newcommand{\yhull}{\hull{y}}
\newcommand{\zhull}{z\ind{h}}
\newcommand{\Nxhull}{N_{x,\mathrm{h}}}
\newcommand{\Nzhull}{N_{z,\mathrm{h}}}
\newcommand{\hullheight}{\hull{y}} 
\newcommand{\shullheight}{\shull{y}}
\newcommand{\elementq}{\varphi}
\newcommand{\structure}{s}

\newcommand{\unitvecx}{\unitvec{x}}
\newcommand{\unitvecy}{\unitvec{y}}
\newcommand{\unitvecz}{\unitvec{z}}

\newcommand{\ttderiv}[1]{\tderiv[2]{#1}}

\usepackage{xparse}

\NewDocumentCommand{\dblavdragacceleration}{o}{%
  \IfNoValueTF{#1}
    {\dragacceleration}
    {{\dragacceleration}_{\!,#1}}
}

\newcommand{\uprelimvec}{\ensuremath{\vectorsym{\uprelim}}}
\newcommand{\collisionforce}{  \relcoll{\vectorsym{\force}} }
\newcommand{\collisiontorque}{ \relcoll{\vectorsym{\torque}} }
\newcommand{\lubricationforce}{  \rellub{\vectorsym{\force}} }
\newcommand{\lubricationtorque}{ \rellub{\vectorsym{m}} }
\newcommand{\dSurface}{\tdiff{S}}
\newcommand{\dVolume}{\tdiff{V}}
\newcommand{\dCurve}{\tdiff{C}}

% fluid structure coupling
\newcommand{\markerarea}{\ensuremath{\Delta{}S}}
\newcommand{\dirac}{\delta}
\newcommand{\codebelow}[2]{ { \color{gray}\underbrace{ \color{black}#1\vphantom{\big|} }_{ \clap{\text{\texttt{#2}}} } } }
\newcommand{\codeabove}[2]{ { \color{gray}\overbrace{  \color{black}#1\vphantom{\big|} }^{ \clap{\text{\texttt{#2}}} } } }
\newcommand{\oldname}[1]{\textcolor{gray}{\sout{#1}}}
\newcommand{\createeqnumber}[1]{\parbox{8mm}{\begin{equation}\label{#1}\end{equation}}}
\newcommand{\zero}[1]{{\color{gray}#1}}
\newcommand{\massspecificforce}{\vectorsym{\force}\ind{m}}
\newcommand{\diracfsinterface}{\delta\relfsinterface}
\newcommand{\planespace}{\omega}
\newcommand{\crosssectionspace}{\Upsilon}

% collision model
\newcommand{\dptot}{\relcoll{\vectorsym{\linmom}}}  % collision impulse
\newcommand{\dptotn}{{\dptot}\ind{n}}
\newcommand{\dptott}{{\dptot}\ind{t}}
\newcommand{\dpv}{\relvelconstr{\vectorsym{\linmom}}}
\newcommand{\dpw}{\relextloads{\vectorsym{\linmom}}}
\newcommand{\distancedir}{\normalvec}
\newcommand{\dnNoncompeting}{\dnLc}
\newcommand{\distNoncompeting}{d\ind{nc}}

\newcommand{\secflow}{\vectorsym{u}_\perp}

==> nomenclature/newcommands.tex <==
% DO NOT MODIFY THIS FILE!
% it was generated by and will be regenerated by pynomencl.

\makeatletter
\newcommand{\adjlength}[0]{x\ind{d}} % adjustment length, 
\newcommand{\angmom}[0]{l} % angular impulse \describevector{\angmom}, 
\newcommand{\angvel}[0]{\omega} % angular velocity \describevector{\angvel}, 
\newcommand{\condaveventarea}[0]{A\condavg} % area associated with an event in the conditional averaging, 
\newcommand{\Archimedes}[0]{\mathit{Ar}} % Archimedes number, 
\newcommand{\arclength}[0]{s} % arc length coordinate, 
\newcommand{\attip}[0]{^{\ast}} % at tip position, 
\newcommand{\bdensity}[0]{\rho\ind{s}} % blade density, 
\newcommand{\bmass}[0]{m\ind{s}} % mass of a blade, 
\newcommand{\bedslope}[0]{S_0} % channel bed slope, 
\newcommand{\bladeA}[0]{A} % cross sectional area of the blade, 
\newcommand{\bladeCg}[1]{c_{\mathrm{s}#1}} % structural damping w.r.t. shearing ($i\in\lbrace1,2\rbrace$) and extension ($i=3$), 
\newcommand{\bladeCk}[1]{c_{\mathrm{b}#1}} % structural damping w.r.t. bending ($i\in\lbrace1,2\rbrace$) and torsion ($i=3$), 
\newcommand{\bladeE}[0]{E\ind{s}} % Young‘s modulus, 
\newcommand{\bladeG}[0]{G\ind{s}} % blade shear  modulus, 
\newcommand{\bladeI}[0]{I} % second moments of area of Cosserat beam (w.r.t. bending), 
\newcommand{\bladeJ}[0]{J} % second polar moment of area of Cosserat beam (w.r.t. twisting), 
\newcommand{\bladeks}[1]{k_{\mathrm{s}#1}} % shear correction factors (w.r.t. cross section axes), 
\newcommand{\bladekt}[0]{k\ind{t}} % correction factor for torsional warping, 
\newcommand{\bladeL}[0]{L\ind{s}} % blade length, 
\newcommand{\bladeLc}[0]{L\ind{c}} % length of a collision element, 
\newcommand{\bladeLcf}[0]{L\ind{f}} % length along which forces on collision element are evaluated, 
\newcommand{\bladeLcm}[0]{L\ind{m}} % length along which torques on collision element are evaluated, 
\newcommand{\bladeLe}[0]{L\ind{e}} % length of a blade element, 
\newcommand{\bladeNe}[0]{N\ind{e}} % number of elements per structure, 
\newcommand{\bladePoissonsratio}[0]{\nu\ind{s}} % Poisson’s ratio, 
\newcommand{\bladeSpacing}[0]{{\Delta}{S}} % distance between the fixed, lower end points of the blades, 
\newcommand{\bladeT}[0]{T\ind{s}} % blade thickness, 
\newcommand{\bladetipvec}[0]{\vectorsym{\ssymbol{x}}^\ast} % location of a blade’s tip, 
\newcommand{\bladetipx}[0]{\ssymbol{x}^\ast} % $y$-coordinate of the location of a blade’s tip, 
\newcommand{\bladetipy}[0]{\ssymbol{y}^\ast} % $y$-coordinate of the location of a blade’s tip, 
\newcommand{\bladetipz}[0]{\ssymbol{z}^\ast} % $z$-coordinate of the location of a blade’s tip, 
\newcommand{\bladeW}[0]{W\ind{s}} % blade width, 
\newcommand{\bladexvec}[0]{\vectorsym{\ssymbol{x}}} % location along a blade relative to its root, $ = \transposed{( \x, \y, \z )}$, 
\newcommand{\BuoyancyNum}[0]{B} % buoyancy number, 
\newcommand{\canopyH}[0]{h} % mean canopy height (average reconfigured height), 
\newcommand{\canopyL}[0]{L\ind{p}} % canopy patch length, 
\newcommand{\distance}[0]{d} % distance vector connecting the contact points in a collision, 
\newcommand{\Cauchy}[0]{\mathit{Ca}} % nominal Cauchy number, 
\newcommand{\CauchyR}[0]{\mathit{Ca}_{\!\ReconfNum}} % Cauchy number computed from $\ReconfNum$, 
\newcommand{\cdensity}[0]{M} % shoots of plants per base area, 
\newcommand{\centerlinepos}[0]{c} % position along the centerline of a structure relative to its root, $\vectorsym{\centerlinepos{}}=\transposed{[\centerlinepos_{x}, \centerlinepos_{y}, \centerlinepos_{z}]}$, 
\newcommand{\surfacepos}[1]{\gamma_{#1}} % position on the surface of a structure relative to its root, $\vectorsym{\surfacepos{}}=\transposed{[\surfacepos{x}, \surfacepos{y}, \surfacepos{z}]}$, 
\newcommand{\CFL}[0]{C\ind{CFL}} % Courant–Friedrichs–Lewy number, 
\newcommand{\channelfx}[0]{f\ind{d}} % Mass-specific channel forcing, 
\newcommand{\channelH}[0]{H} % height of simulation domain, 
\newcommand{\channelL}[0]{L_x} % length of simulation domain, 
\newcommand{\channelW}[0]{L_z} % width of simulation domain, 
\newcommand{\circconv}[2]{#1 \mathbin{\circledast} #2} % circular convolution of $a$ and $b$, 
\newcommand{\bcdot}[0]{\mathbin{\boldsymbol{\cdot}}} % Scalar product or matrix product, 
\newcommand{\restitutioncoefficient}[0]{{c\ind{e}}} % coefficient of restitution, 
\newcommand{\condavg}[0]{_{{\mathrm{c}}}} % related to the conditional average, 
\newcommand{\condav}[1]{\mleft\langle #1 \mright\rangle\ind{c}} % conditional average, 
\newcommand{\corr}[2]{\rho_{#1#2}} % correlation coefficient of $p$ and $q$, 
\newcommand{\critfrictionvelocity}[0]{u_{\ast\mathrm{crit}}} % critical friction velocity, 
\newcommand{\critroughnessdensity}[0]{\roughnessdensity\ind{t}} % threshold roughness density, 
\newcommand{\crosssectiontensorofinertia}[0]{\tensorsym{I}} % tensor of inertia of Cosserat beam cross sections (second moments of area), 
\newcommand{\Csmag}[0]{C\ind{S}} % smagorinsky coefficient, 
\newcommand{\dampingratio}[0]{\zeta} % damping ratio, 
\newcommand{\darclength}[0]{{\mathsmaller\Delta}{\arclength}} % arc length of an element, 
\newcommand{\ddensity}[0]{{\mathsmaller\Delta}\rho} % $=\fdensity-\bdensity$, 
\newcommand{\deltafunction}[1]{\Phi_{#1}} % $n$-point regularized delta function, 
\newcommand{\developmentlength}[0]{x_\ast} % Development length \cite{ChenFlow2013}, 
\newcommand{\DIF}[0]{\mathit{DIF}} % Diffusion number, 
\newcommand{\displheight}[0]{y\ind{vo}} % Virtual origin, zero-displacement height, lower limit for effective overflow, NepfFlow2000
\newcommand{\dblav}[1]{\lrangles*{#1}} % double average (in time and periodic directions), 
\newcommand{\tav}[2][t]{\lrangles*{#2}_{#1}} % time average, 
\newcommand{\sav}[2][xz]{\lrangles*{#2}_{#1}} % spatial average (along the directions, indicated, e.g.~$x$, $z$), 
\newcommand{\tfl}[1]{#1^{\prime}\mkern-1.2mu} % fluctuations from time average, 
\newcommand{\sfl}[1]{#1^{\prime\mkern-1.2mu\prime}\mkern-1.2mu} % fluctuations from spatial average, 
\newcommand{\dOne}[0]{\vectorsym{d}_1} % unit vector in the direction along which the width of the blade is measured, 
\newcommand{\dragcoeff}[0]{C\ind{d}} % drag coefficient, 
\newcommand{\dragforce}[0]{F\ind{d}} % drag force, 
\newcommand{\dragacceleration}[0]{f\ind{v}} % mass-specific force vector due to vegetation drag, 
\newcommand{\draglength}[0]{L\ind{d}} % drag length scale, CocealCanopy2004
\newcommand{\dt}[0]{{\mathsmaller\Delta}t} % time step size, 
\newcommand{\dThree}[0]{\vectorsym{d}_3} % unit vector tangential to the skeleton of the blade, 
\newcommand{\dTwo}[0]{\vectorsym{d}_2} % unit vector in the direction along which the thickness of the blade is measured, 
\newcommand{\celledgelength}[0]{\Delta\ind{g}} % mean edge length of computational grid, 
\newcommand{\dx}[0]{\Delta_x} % cell width of computational grid, 
\newcommand{\dy}[0]{\Delta_y} % cell height of computational grid, 
\newcommand{\dz}[0]{\Delta_z} % cell depth of computational grid, 
\newcommand{\eind}[0]{_{\mathrm{e}}} % related to an element, 
\newcommand{\externalforcedensity}[0]{\vectorsym{{\accsmalltriangledown{f}}}} % arc-length-specific external force, 
\newcommand{\gravityforcedensity}[0]{\vectorsym{\accsmalltriangledown{f}_\grav}} % arc-length-specific external force due to gravity, 
\newcommand{\externaltorquedensity}[0]{\vectorsym{{\accsmalltriangledown{m}}}} % arc-length-specific external torque, 
\newcommand{\fapv}[0]{a} % frontal area per canopy volume, 
\newcommand{\fdensity}[0]{\rho} % density of the fluid, 
\newcommand{\find}[0]{_{\mathrm{f}}} % related to the fluid, 
\newcommand{\fluidlayerheight}[0]{h} % height of fluid layer associated with zero-thickness blade interface, 
\newcommand{\fluidvolumespace}[0]{\Omega\ind{f}} % fluid volume space, $ \fluidvolumespace\subset\wholespace$, 
\newcommand{\force}[0]{f} % force \describevector{\force}, 
\newcommand{\forceacceleration}[0]{f} % mass-specific force, 
\newcommand{\forcingcrosssectionspace}[0]{\lambda} % plain section of $\forcingvolumespace$, co-planar with $\structurecrosssectionspace$, 
\newcommand{\forcingcrosssectiontensorofinertia}[0]{\tensorsym{{\tilde{I}}}} % tensor of inertia of fluid layer cross section due to fluid-structure coupling, 
\newcommand{\forcingtensorofinertia}[0]{\tensorsym{{\tilde{J}}}} % tensor of inertia of fluid layer due to fluid-structure coupling, 
\newcommand{\forcingvolumespace}[0]{\Lambda} % fluid layer surrounding $\fsinterface$ where forcing takes place, $\forcingvolumespace\subset\fluidvolumespace$, 
\newcommand{\frictionvelocity}[0]{u_{\tau}} % friction velocity, 
\newcommand{\frictionvelocityin}[0]{u_{\tau,\mathrm{i}}} % inner friction velocity based on the wall shear stress at the canopy bed, 
\newcommand{\frictionvelocityloc}[0]{u_{\tau,\mathrm{l}}} % local friction velocity, 
\newcommand{\frictionvelocityout}[0]{u_{\tau,\mathrm{o}}} % outer (global) friction velocity, 
\newcommand{\roughnessfunction}[0]{\Delta{}U^+} % roughness function in the displaced logarithmic law, 
\newcommand{\viscouslength}[0]{\ell_\tau} % viscous length in the logarithmic law of the wall, 
\newcommand{\Froude}[0]{\mathit{Fr}} % Froude number, 
\newcommand{\fsinterface}[0]{\Gamma} % fluid-structure interface, 
\newcommand{\meantipheight}[0]{h^\ast} % mean tip height, 
\newcommand{\fsinterfacesectionspace}[0]{\gamma} % line section of the fluid-structure interface, $\fsinterfacesectionspace\subset\fsinterface$, 
\newcommand{\Galilei}[0]{\mathit{Ga}} % Galilei number, 
\newcommand{\grav}[0]{g} % gravity and its magnitude $\vectorsym{g}=\transposed{(\grav_x,\grav_y,\grav_z)}$, 
\newcommand{\hlog}[0]{\ylog} % lower limit of the log-law zone, SanjouTurbulence2016
\newcommand{\ylog}[0]{y\ind{log}} % lower limit of the log-law zone, 
\newcommand{\hull}[1]{\widetilde{#1}} % Canopy-hull projection of $\varphi$, 
\newcommand{\hydraulicdiameter}[0]{D} % hydraulic diameter, 
\newcommand{\shull}[1]{\overbar{#1}} % smoothed canopy-hull projection of $\varphi$, 
\newcommand{\identity}[0]{\matrixsymconst{I}} % identity matrix, $\identity=\diag(1)$, 
\newcommand{\internalforce}[0]{\accsmalltriangleup{f}} % internal force of Cosserat beam \describevector{\internalforce}, 
\newcommand{\internaltorque}[0]{\accsmalltriangleup{m}} % internal torque of Cosserat beam \describevector{\internaltorque}, 
\newcommand{\IntOp}[0]{\vectorsym{\mathcal{I}}} % interpolation operator, 
\newcommand{\inversequaternionmatrixofinertia}[0]{\matrixsym{\mathcal{M}}} % \enquote{tangential inverse} quaternion matrix of inertia, 
\newcommand{\kinvis}[0]{\nu} % kinematic viscosity of the fluid, 
\newcommand{\linmom}[0]{p} % linear impulse \describevector{\linmom}, 
\newcommand{\mass}[0]{m} % mass (of colliding structure segment $\relcoll{\mass}$, of marker point $\relmarker{\mass}$, …), 
\newcommand{\relelement}[2]{#1_{#2}} % related to the $n$th structure, structure element, collision element, or the $n$th Lagrangian marker (also applied to an entire expression in the form $\relelement{[\dots]}{n}$), 
\newcommand{\relrkstep}[2]{#1^{(#2)}} % value at the $r$th time step or Runge Kutta step, 
\newcommand{\skeletonvector}[0]{\vectorsym{e\ind{s}}} % skeleton vector, $\vnorm{\skeletonvector}=1$, 
\newcommand{\mixinglength}[0]{L\ind{ml}} % vertical mixing length, 
\newcommand{\mixinglthness}[0]{t\ind{ml}} % mixing layer thickness, 
\newcommand{\mixinglU}[0]{U\ind{ml}} % mean velocity in the mixing layer, HoPerturbed1984
\newcommand{\mixinglUdiff}[0]{{\mathsmaller\Delta}U\ind{ml}} % mean velocity difference in the mixing layer, HoPerturbed1984
\newcommand{\momentumthness}[0]{\theta} % momentum thickness, 
\newcommand{\nBlades}[0]{N\ind{s}} % number of structures, 
\newcommand{\nCells}[0]{N} % number of cells, $\nCells=\nCells_x  \nCells_y \nCells_z$, 
\newcommand{\nMarkers}[0]{N\ind{l}} % number of forcing points, 
\newcommand{\insurface}[1]{#1_\parallel} % surface-parallel components of a vector ($\insurface{\vectorsym{u}}\coloneqq \vectorsym{u} - (\vectorsym{u}\bcdot\vectorsym{n})\vectorsym{n}$), 
\newcommand{\patternLength}[0]{L\ind{p}} % length of blade placement, 
\newcommand{\pdf}[1]{\phi_{#1}} % probability density function of a variable $\varphi$, 
\newcommand{\cdf}[1]{\Phi_{#1}} % cumulative distribution function of a variable $\varphi$, 
\newcommand{\penetrationdepth}[0]{\delta\ind{e}} % penetration depth, 
\newcommand{\penetrationheight}[0]{h\ind{p}} % penetration height, NepfFlow2000
\newcommand{\percentile}[2]{P_{#1}\of{#2}} % $p$-percentile of $b$, 
\newcommand{\pre}[0]{\tilde{\pressure}} % modified pressure, 
\newcommand{\pressure}[0]{p} % pressure, 
\newcommand{\qcdot}[0]{\mathbin{\ast}} % multiplication of two quaternions $\vectorsym{a}$, $\vectorsym{b}$ (non-commutative), 
\newcommand{\dyaddot}[0]{\mathbin{\otimes}} % dyadic (tensor) product of two vectors $\vectorsym{a}$, $\vectorsym{b}$, 
\newcommand{\qconj}[1]{\overline{#1}} % conjugate of a quaternion $\quaternion$, 
\newcommand{\qimag}[1]{\vectorsym{\mathrm{Im}}\of{#1}} % imaginary part of a quaternion $\quaternion$, 
\newcommand{\qreal}[1]{\mathrm{Re}\of{#1}} % real part of a quaternion $\quaternion$, 
\newcommand{\conj}[1]{#1^\ast} % conjugate of a complex number, 
\newcommand{\quaternion}[0]{\vectorsym{q}} % quaternion, 
\newcommand{\quaternionmatrix}[0]{\matrixsym{\mathcal{Q}}} % quaternion matrix, 
\newcommand{\quaternionmatrixofinertia}[0]{\matrixsym{\mathcal{I}}_0} % quaternion matrix of inertia, 
\newcommand{\ReconfNum}[0]{R} % reconfiguration number, 
\newcommand{\reconfW}[0]{W^\ast} % mean plant width perpendicular to the mean flow, 
\newcommand{\relvo}[2][]{#2_{#1\mathrm{vo}}} % related to the virtual origin of the outer flow, 
\newcommand{\relinner}[1]{#1\ind{i}} % related to inner (wall) units, 
\newcommand{\relcoll}[1]{#1\ind{c}} % related to collision, 
\newcommand{\relmarker}[2][]{{#2_\mathrm{m}}_{#1}} % related to an IBM marker point, 
\newcommand{\relextloads}[1]{#1\ind{w}} % due to external loads, 
\newcommand{\relfsinterface}[0]{_{\mathit{\Gamma}}} % related to the fuid-stucture interface, 
\newcommand{\relgravity}[1]{#1\ind{g}} % due to gravity, 
\newcommand{\rellub}[1]{#1\ind{lub}} % due to lubrication, 
\newcommand{\releff}[1]{#1\ind{eff}} % effective quantity which includes inertial part of fluid structure forcing, 
\newcommand{\relpos}[0]{\xi} % position relative to center of structure crosssection (analytical description) or nearest element center (discretized) \describevector{\relpos}, 
\newcommand{\relref}[1]{#1\ind{0}} % in the reference configuration, 
\newcommand{\relvelconstr}[1]{#1\ind{v}} % due to velocity constraint, 
\newcommand{\Reynolds}[0]{\mathit{Re}} % Reynolds number, 
\newcommand{\rotationmatrix}[0]{\matrixsym{R}} % rotation matrix, 
\newcommand{\roughnessdensity}[0]{\lambda} % frontal plant area per bed area, WoodingDrag1973, NepfFlow2012
\newcommand{\roughnessheight}[0]{y_0} % roughness length \cite[p.\,552]{NepfFlow2000}, NepfFlow2000
\newcommand{\sgsstress}[0]{\tensorsym{\tau}\ind{sgs}} % subgrid-scale stress tensor, 
\newcommand{\sgsvis}[0]{\nu\ind{sgs}} % subgrid-scale viscosity, 
\newcommand{\thresholdyLo}[0]{\sfl{y}\ind{c,t}} % threshold value identifying trough events, 
\newcommand{\thresholdyHi}[0]{\sfl{y}\ind{c,r}} % threshold value identifying ridge events, 
\newcommand{\condavSetLo}[0]{\mathcal{C}\ind{t}} % set of valley events, 
\newcommand{\condavSetHi}[0]{\mathcal{C}\ind{r}} % set of ridge events, 
\newcommand{\condavR}[0]{R\condavg} % radius in which a trigger event shall be the extremum, 
\newcommand{\critarea}[0]{A\ind{crit}} % minimum area of a trigger event, 
\newcommand{\Sh}[0]{S} % strain rate tensor, 
\newcommand{\ShearLengthScale}[0]{L\ind{s}} % shear length scale, 
\newcommand{\shearstress}[0]{\tau} % shear stress \describevector{\shearstress}, 
\newcommand{\shearstressint}[0]{\widetilde{\shearstress}} % total shear stress (in double averaged framework), including canopy drag, 
\newcommand{\sind}[0]{_{\mathrm{s}}} % related to a structure, 
\newcommand{\skewmatrix}[1]{\left[#1\right]_\times} % skew matrix of a vector $\vectorsym{a}$: $\skewmatrix{\vectorsym{a}}\bcdot\vectorsym{b} = \vectorsym{a}\times\vectorsym{b}$, 
\newcommand{\slope}[0]{S} % channel slope, 
\newcommand{\psd}[1]{\Phi_{#1#1}} % power spectral density of a variable $\varphi$, 
\newcommand{\copsd}[2]{\Phi_{#1#2}} % co-power spectral density of two variables $u$, $v$, 
\newcommand{\Spr}[0]{\vectorsym{\mathcal{S}}} % spreading operator, 
\newcommand{\statevec}[0]{\vectorsym{z}} % state vector, 
\newcommand{\Strouhal}[0]{\mathit{St}} % Strouhal number, 
\newcommand{\structurecrosssectionspace}[0]{\Upsilon} % plain cross section of the structure volume $\structurevolumespace$, 
\newcommand{\structurevolumespace}[0]{\Omega\ind{s}} % structure volume space, $\structurevolumespace\subset\wholespace$, 
\newcommand{\substep}[0]{k} % substep counter, 
\newcommand{\surfH}[0]{H} % water level height (including canopy), 
\newcommand{\surfwavelength}[0]{\lambda^\ast} % wavelength of the canopy surface, 
\newcommand{\surfwavelengthx}[0]{\lambda^\ast_x} % wavelength of the canopy surface in $x$-direction, 
\newcommand{\wavelength}[0]{\lambda} % wavelength (in $x$-direction), 
\newcommand{\svf}[0]{\lambda\ind{p}} % solid volume fraction, plantform density, MandelSurface2019
\newcommand{\tensorofinertia}[0]{\tensorsym{J}} % tensor of inertia, 
\newcommand{\timestep}[0]{n} % time step counter, 
\newcommand{\tke}[0]{K} % instantaneous turbulence kinetic energy, 
\newcommand{\torque}[0]{m} % torque \describevector{\torque}, 
\newcommand{\trace}[0]{\mathrm{tr}} % trace of a matrix $\matrixsym{A}$, 
\newcommand{\transposed}[1]{#1^\top} % transposed of vector $\vectorsym{a}$ or matrix $\matrixsym{A}$, 
\newcommand{\ubulk}[0]{U} % bulk velocity, 
\newcommand{\unitvec}[1]{\vectorsym{e}_{#1}} % unit vector in streamwise, vertical and spanwise direction, respectively, 
\newcommand{\uprelim}[0]{\tilde{\vel}} % preliminary fluid velocity vector (after the explicit RK step), 
\newcommand{\vel}[0]{u} % fluid velocity vector, 
\newcommand{\volumeforcevec}[0]{\vectorsym{f}\ind{V}} % volume force vector, 
\newcommand{\vonKarmanConst}[0]{\kappa} % von Kármán constant (velocity log-law), 
\newcommand{\wavenumber}[0]{\kappa} % wavenumber (in $x$-direction), 
\newcommand{\vortexh}[0]{h\ind{v}} % vortex core height, GhisalbertiMixing2002
\newcommand{\vortexU}[0]{U\ind{v}} % vortex velocity, GhisalbertiMixing2002
\newcommand{\WakeLengthScale}[0]{L\ind{w}} % wake (vortex shedding) length scale, 
\newcommand{\wallshear}[0]{\tau\ind{w}} % wall shear stress vector \describevector{{\wallshear}}, 
\newcommand{\wholespace}[0]{\Omega} % entire physical domain, $\wholespace = \structurevolumespace\cup\fluidvolumespace$, 
\newcommand{\wholespacesection}[0]{\omega} % plain section of the physical domain, extending a structure cross section, $\structurecrosssectionspace\subset\wholespacesection$, 
\newcommand{\xvec}[0]{\vectorsym{x}} % position vector, $\vectorsym{x}=\transposed{(x,y,z)}$, 
\newcommand{\ylip}[0]{y\ind{lip}} % height of lower inflection point in profile of mean streamwise velocity, 
\newcommand{\yuip}[0]{y\ind{uip}} % height of upper inflection point in profile mean streamwise velocity, 
\newcommand{\Tst}[0]{T\ind{st}} % duration of startup phase, 
\newcommand{\Tav}[0]{T\ind{av}} % duration of sampling phase, 
\newcommand{\Tavspace}[0]{\Omega_{T\ind{av}}} % time space during which statistics are collected, 
\newcommand{\xzspace}[0]{\Omega_{xz}} % horizontal space spanned by $\unitvecx$ and $\unitvecz$, 
\newcommand{\condavSet}[0]{\mathcal{C}} % set of conditional events, 
\newcommand{\Rspace}[0]{\Omega_R} % horizontal, circular space within radius $R$ of an event, 
\newcommand{\condavspace}[0]{\Omega\condavg} % connected region of $\xzspace$ associated with an event, 
\newcommand{\forceoncollisionelement}[0]{\vectorsym{\tilde{f}}} % force acting on collision element, 
\newcommand{\torqueoncollisionelement}[0]{\vectorsym{\tilde{m}}} % torque acting on collision element, 
\newcommand{\forcingcrosssectionarea}[0]{\tilde{A}} % cross sectional area of forcing range, 
\newcommand{\modexternalforcedensityrelfsinterface}[0]{\vectorsym{\tilde{\accsmalltriangledown{f}}_\mathit{\!\Gamma}}} % explicit part of arc-length-specific force due to fluid-sructure coupling, 
\newcommand{\modexternaltorquedensityrelfsinterface}[0]{\vectorsym{\tilde{\accsmalltriangledown{m}}_\mathit{\!\Gamma}}} % explicit part of arc-length-specific torque due to fluid-sructure coupling, 
\newcommand{\externalforcedensityrelfsinterface}[0]{\vectorsym{\accsmalltriangledown{f}_\mathit{\!\Gamma}}} % arc-length-specific force due to fluid-sructure coupling, 
\newcommand{\externaltorquedensityrelfsinterface}[0]{\vectorsym{\accsmalltriangledown{m}_\mathit{\!\Gamma}}} % arc-length-specific torque due to fluid-sructure coupling, 
\newcommand{\hydrodynamicstress}[0]{\sigma} % hydrodynamic stress tensor, 
\newcommand{\ddry}[0]{d\ind{dry}} % security distance in collision model, 
\newcommand{\dlub}[0]{d\ind{lub}} % lubrication distance in collision model, 
\newcommand{\dsph}[0]{d\ind{sph}} % gap distance between enveloping spheres in collision model, 
\newcommand{\npartners}[0]{N\ind{max}} % upper bound for number of colliding other elements, 
\newcommand{\Rsph}[0]{R} % radius of an enveloping sphere, 
\newcommand{\dcrit}[0]{d\ind{crit}} % critical distance in collision model, 
\newcommand{\dnLc}[0]{n\ind{ce}} % number of structure elements per collision element, 
\newcommand{\tderiv}[2][1]{\ifthenelse{\equal{#1}{1}}{\dot{#2}}{%
\ifthenelse{\equal{#1}{2}}{\ddot{#2}}{%
\ifthenelse{\equal{#1}{3}}{\dddot{#2}}{%
\ifthenelse{\equal{#1}{4}}{\ddddot{#2}}{%
\frac{\partial^#1#2}{\partial t^#1}}}}}} % temporal derivative of $a$ (first, second, \ldots), 
\newcommand{\sderiv}[1]{#1’} % spatial derivative of $a$, 1D derivative in structure equations, 
\newcommand{\relpside}[1]{#1\Ind{+}} % related to one side of the interface, 
\newcommand{\relmside}[1]{#1\Ind{-}} % related to other side of the interface, 
\newcommand{\relwallunits}[1]{#1\Ind{+}} % quantity scaled in wall units, 
\newcommand{\relwallunitsvo}[1]{#1\Ind{+,vo}} % quantity scaled in wall units of the overflow, related to the displacement height $\displheight$, 
\newcommand{\normalvec}[0]{\vectorsym{n}} % unit vector normal to interface, 
\newcommand{\postcollision}[1]{#1’} % quantity after collision, 
\newcommand{\diraccollision}[0]{\delta\ind{c}} % dirac delta function associated with a collision impulse, 
\newcommand{\systemmatrix}[0]{\matrixsym{K}} % system matrix relating collision impulse to the change of relative velocity, 
\newcommand{\cpvel}[0]{v} % velocity of a contact point, 
\newcommand{\dvtot}[0]{\Delta{}\vectorsym{v}} % change of relative velocity due to collision impulse, 
\newcommand{\frictioncoeffstatic}[0]{\mu\ind{s}} % coefficient of static friction, 
\newcommand{\frictioncoeffdynamic}[0]{\mu\ind{k}} % coefficient of dynamic friction, 
\newcommand{\gapdistance}[0]{d\ind{g}} % gap distance between canopy blades, 
\newcommand{\orderof}[1]{\mathcal{O}\of{#1}} % Landau symbol, 
\newcommand{\reducedvelocity}[0]{U\ind{r}} % reduced velocity, 
\newcommand{\naturalfrequency}[0]{f\ind{n}} % Natural frequency of a blade, 
\newcommand{\vorticity}[0]{\omega} % vorticity vector \describevector{\vorticity}, 
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor} % floor to closest integer, 
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil} % ceil to closest integer, 
\newcommand{\strain}[0]{\varepsilon} % strain vector of the Cosserat rod centerline, 
\newcommand{\curvature}[0]{\kappa} % curvature vector of the Cosserat rot centerline, 
\newcommand{\FT}[0]{\mathcal{F}} % Fourier transform, 
\newcommand{\volumefraction}[0]{\alpha} % volume fraction occupied by the canopy elements, 
\newcommand{\lambdatwo}[0]{\lambda_2} % $\lambdatwo$ vortex criterion of the velocity vector $\vectorsym{u}$, 
\newcommand{\submersion}[0]{\Pi\ind{h}} % level of submersion, 
\newcommand{\basearea}[0]{A\ind{s}} % floor area per blade, 
\newcommand{\addedmasscrosssection}[0]{A\ind{a}} % cross sectional area determining the added mass, 
\newcommand{\addedmass}[0]{m\ind{a}} % added mass, 
\newcommand{\timevar}[0]{t} % time, 
\newcommand{\nModes}[0]{N\ind{n}} % number of nodes in modal reconstruction of blade motion, 
\newcommand{\jpdf}[2]{\phi_{#1,#2}} % Joint probability density function of the variables $\varphi$, $\vartheta$, 
\newcommand{\rhsvecforce}[0]{\vectorsym{r\ind{f}}} % right-hand side of equation for translational velocity of Cosserat rod, 
\newcommand{\rhsvecomega}[0]{\vectorsym{r}_{\!\omega}} % right-hand side of equation for anglular velocity of Cosserat rod, 
\newcommand{\rhsvecquaternion}[0]{\vectorsym{r\ind{q}}} % right-hand side of equation for quaternional velocity of Cosserat rod, 
\newcommand{\volumecouplingforce}[0]{f_\mathit{\!\Gamma}} % volume force resulting from fluid-structure coupling, 
\newcommand{\surfacecouplingforce}[0]{\vectorsym{f\ind{s}}} % surface-specific force from fluid-structure coupling, 
\newcommand{\setofelements}[0]{\Omega\ind{e}} % set of all structure elements, of elements belonging to $s$th structure, 
\newcommand{\contactpointvec}[0]{\vectorsym{r}} % vector from element center to contact point, 
\newcommand{\vrelvecv}[0]{\relvelconstr{\vectorsym{v}}} % relative velocity of the contact points (before collision), 
\newcommand{\vrelvecw}[0]{\relextloads{\Delta\vectorsym{v}}} % change of relative velocity of contact points due to loads on collision elements, 
\newcommand{\forcingmass}[0]{\tilde{m}} % mass associated with the marker points on a blade element, 
\newcommand{\forcinginertialmoment}[0]{\tilde{s}} % static moment of fluid layer mass, 
\newcommand{\retardationtimee}[0]{\tau\ind{e}} % retardation time for extension, 
\newcommand{\retardationtimes}[0]{\tau\ind{s}} % retardation time for shearing, 
\newcommand{\Cstrainrate}[0]{\matrixsym{C}_{\dot{\strain}}} % constitutive matrix w.r.t. strain rate vector $\vectorsym{\dot{\strain}}$, 
\newcommand{\Cstrain}[0]{\matrixsym{C}_{\strain}} % constitutive matrix w.r.t. strain vector $\vectorsym{\strain}$, 
\newcommand{\Ccurvature}[0]{\matrixsym{C}_{\curvature}} % constitutive matrix w.r.t. curvature vector $\vectorsym{\curvature}$, 
\newcommand{\Ccurvaturerate}[0]{\matrixsym{C}_{\dot{\curvature}}} % constitutive matrix w.r.t. curvature rate vector $\vectorsym{\dot{\curvature}}$, 
\newcommand{\CollPairsNC}[0]{\mathcal{P}\ind{\!nc}} % set of \enquote{non-competing} collision pairs, 
\newcommand{\CollPairs}[0]{\mathcal{P}} % set of collision pairs, 
\newcommand{\resolvedTKERatio}[0]{Q_K} % ratio of resolved turbulence kinetic energy, 
\newcommand{\CelikEtaIndex}[0]{Q_\eta} % single-grid estimator for LES grid resolution quality based on estimated Kolmogorov scale, 
\newcommand{\CelikNuIndex}[0]{Q_\nu} % single-grid estimator for LES grid resolution quality based on relative effective viscosity, 
\newcommand{\sgsactivity}[0]{Q_\varepsilon} % sub-grid stress activity, 
\makeatother

% Included from customcommands.tex

%\usepackage{relsize}

%%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%% Gray rectangle to illustrate the use of modifiers and indices
%%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%\usepackage{stix} % provides \vrectangleblack, but clashes with other packages
%\usepackage{ifsym}
%\newcommand{\vgbox}{\text{\textcolor{gray}{\FilledSmallSquare}}}

%\DeclareFontFamily{U}{MnSymbolC}{}
%\DeclareFontShape{U}{MnSymbolC}{m}{n}{
%	<-5.5> MnSymbolC5
%	<5.5-6.5> MnSymbolC6
%	<6.5-7.5> MnSymbolC7
%	<7.5-8.5> MnSymbolC8
%	<8.5-9.5> MnSymbolC9
%	<9.5-11.5> MnSymbolC10
%	<11.5-> MnSymbolCb12
%}{}
%\DeclareRobustCommand{\gsqcdot}{%
%	\mathbin{\text{\color{gray}\usefont{U}{MnSymbolC}{m}{n}\symbol{"69}}}%
%}

%\newcommand{\gsqcdot}{\text{\color{gray}\filledsquare}}

%%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~
%% Some custom commands
%%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~

\newcommand{\describevector}[1]{$\vectorsym{#1} = \transposed{(#1_x, #1_y, #1_z)}$}

%\newcommand{\SymbolForIllustrationOfScripts}{\cdot}
%\newcommand{\SymbolForIllustrationOfScripts}{(\cdot)}
\newcommand{\SymbolForIllustrationOfScripts}{\raisebox{-1pt}{$\color{gray}\blacksquare$}}
\newcommand{\wildcard}{\cdot}
\newcommand{\pwildcard}{(\cdot)}

%\DeclareMathAlphabet{\mathsfit}{T1}{\sfdefault}{\mddefault}{\sldefault}
%\SetMathAlphabet{\mathsfit}{bold}{T1}{\sfdefault}{\bfdefault}{\sldefault}
\newcommand{\s}{\mathrm{s}}
%\newcommand{\ssymbol}[1]{#1}
%\newcommand{\Deltadiff}[1]{{\Delta\!\!\:#1}}

% Commands for 2-column nomenclature layout
%\renewcommand*{\nompreamble}{\begin{multicols}{2}}
%	\renewcommand*{\nompostamble}{\end{multicols}}
%\setlength{\columnseprule}{0.4pt}

\newcommand{\ssymbol}[1]{\mathsfit{#1}}

% https://tex.stackexchange.com/a/712336/63717
\usepackage{amsmath,mathtools}
\DeclarePairedDelimiter{\anglebrackets}{\langle}{\rangle}
\NewDocumentCommand{\lrangles}{some{_^}}{%
  \IfBooleanTF{#1}{% *
    \anglebrackets*{#3}%
    \IfValueT{#4}{_{\!#4}}% subscript
    \IfValueT{#5}{^{\!#5}}% superscript
  }{%
    \IfNoValueTF{#2}{%
      \anglebrackets{#3}%
      \IfValueT{#4}{_{#4}}% subscript
      \IfValueT{#5}{^{#5}}% superscript
    }{%
      \anglebrackets[#2]{#3}%
      \IfValueT{#4}{_{\!#4}}% subscript
      \IfValueT{#5}{^{\!#5}}% superscript
    }%
  }%
}


% =======================================================

\newcommand{\structureelement}{n}
\newcommand{\collisionelement}{n}
\newcommand{\masterelement}{n}
\newcommand{\markerelement}{l}
\newcommand{\relstructureelement}[2]{\relelement{#1}{#2}}
\newcommand{\relcollisionelement}[2]{\relelement{#1}{#2}}
\newcommand{\relmarkerelement}[2]{\relelement{#1}{#2}}
\renewcommand{\gravityforcedensity}{\relgravity{\externalforcedensity}}
\newcommand{\bladekOne}{\bladeks{1}}
\newcommand{\bladekTwo}{\bladeks{2}}
\newcommand{\rkstep}{r}
%\introducerelrkstep
%\newcommand{\jpdf}[2]{\pdf{#1,#2}}
%\newcommand{\forcingmass}{\tilde{m}}

\newcommand{\collisionelementmass}{\relcoll{\mass}}
\newcommand{\markermass}{\relmarker{\mass}}


\newcommand{\frictionvelocityvo}{\relvo[\!,]{{\frictionvelocity}}}
\newcommand{\roughnessfunctionvo}{\relvo{\roughnessfunction}}
\newcommand{\viscouslengthvo}{\relvo{{\viscouslength}}}
\newcommand{\Reynoldsvo}{\relvo[\!,]{{\Reynolds_\tau}}}
\newcommand{\yplus}{y^+}

\newcommand{\imag}{\mathrm{i}}
\newcommand{\e}{\mathrm{e}}

\newcommand{\x}{\centerlinepos_x}
\newcommand{\y}{\centerlinepos_y}
\newcommand{\z}{\centerlinepos_z}
\newcommand{\negcorrxy}{-\corr{\tfl{\x}}{\tfl{\y}}}
\newcommand{\turbfrequency}{f\ind{t}}
\newcommand{\flapfrequency}{f\ind{f}}

\newcommand{\xhull}{x\ind{h}}
\newcommand{\yhull}{\hull{y}}
\newcommand{\zhull}{z\ind{h}}
\newcommand{\Nxhull}{N_{x,\mathrm{h}}}
\newcommand{\Nzhull}{N_{z,\mathrm{h}}}
\newcommand{\hullheight}{\hull{y}} 
\newcommand{\shullheight}{\shull{y}}
\newcommand{\elementq}{\varphi}
\newcommand{\structure}{s}

\newcommand{\unitvecx}{\unitvec{x}}
\newcommand{\unitvecy}{\unitvec{y}}
\newcommand{\unitvecz}{\unitvec{z}}

\newcommand{\ttderiv}[1]{\tderiv[2]{#1}}

\usepackage{xparse}

\NewDocumentCommand{\dblavdragacceleration}{o}{%
  \IfNoValueTF{#1}
    {\dragacceleration}
    {{\dragacceleration}_{\!,#1}}
}

\newcommand{\uprelimvec}{\ensuremath{\vectorsym{\uprelim}}}
\newcommand{\collisionforce}{  \relcoll{\vectorsym{\force}} }
\newcommand{\collisiontorque}{ \relcoll{\vectorsym{\torque}} }
\newcommand{\lubricationforce}{  \rellub{\vectorsym{\force}} }
\newcommand{\lubricationtorque}{ \rellub{\vectorsym{m}} }
\newcommand{\dSurface}{\tdiff{S}}
\newcommand{\dVolume}{\tdiff{V}}
\newcommand{\dCurve}{\tdiff{C}}

% fluid structure coupling
\newcommand{\markerarea}{\ensuremath{\Delta{}S}}
\newcommand{\dirac}{\delta}
\newcommand{\codebelow}[2]{ { \color{gray}\underbrace{ \color{black}#1\vphantom{\big|} }_{ \clap{\text{\texttt{#2}}} } } }
\newcommand{\codeabove}[2]{ { \color{gray}\overbrace{  \color{black}#1\vphantom{\big|} }^{ \clap{\text{\texttt{#2}}} } } }
\newcommand{\oldname}[1]{\textcolor{gray}{\sout{#1}}}
\newcommand{\createeqnumber}[1]{\parbox{8mm}{\begin{equation}\label{#1}\end{equation}}}
\newcommand{\zero}[1]{{\color{gray}#1}}
\newcommand{\massspecificforce}{\vectorsym{\force}\ind{m}}
\newcommand{\diracfsinterface}{\delta\relfsinterface}
\newcommand{\planespace}{\omega}
\newcommand{\crosssectionspace}{\Upsilon}

% collision model
\newcommand{\dptot}{\relcoll{\vectorsym{\linmom}}}  % collision impulse
\newcommand{\dptotn}{{\dptot}\ind{n}}
\newcommand{\dptott}{{\dptot}\ind{t}}
\newcommand{\dpv}{\relvelconstr{\vectorsym{\linmom}}}
\newcommand{\dpw}{\relextloads{\vectorsym{\linmom}}}
\newcommand{\distancedir}{\normalvec}
\newcommand{\dnNoncompeting}{\dnLc}
\newcommand{\distNoncompeting}{d\ind{nc}}

\newcommand{\secflow}{\vectorsym{u}_\perp}
